Analysis of core-mantle boundary seismic waves using full\-waveform modelling and adjoint methods

Using spectral-element and adjoint methods, we investigate body waves interacting with the Earth's most dramatic interface, the core-mantle boundary (CMB). Intermediate-to-high frequency seismograms are computed incorporating topography models. We analyse the sensitivity of many seismic phases interacting with the interface. The study aims at showing effects of CMB structure on synthetics and highlights difficulties of imaging this region due to strong trade-off between velocity variations and topography. Synthetic waveforms computed at dominant periods of 6-18 seconds are used in order to observe time shifts due to topography and calculate the adjoint sensitivity kernel. We focus on diffracted, core reflected and refracted P and S waves. The sensitivity kernel depicts first Fresnel zones of these phases and others that may contribute to narrow time window, although unpredicted by ray theory. We perform comparisons between time shifts due to topography models made on full-waveform synthetics to ray theoretical predictions to assess methods usually deployed for imaging CMB. This shows that for most phases ray theory performs well enough with some accuracy loss. We propose that using relevant seismic phases simultaneously in full-waveform inversion may improve CMB topography imaging. However, it seems necessary to jointly invert for velocity variations due to D\" layer, which is so far poorly understood and presents a challenge when it comes to identifying its effects on traveltime data. In our further research, a FWI workflow is being developed and aims at addressing these issues.

==> figures.tex <==

\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth, angle=90]{figures/curvesCMB}
    \caption{\textit{Left}: Traveltime curves according to model PREM and TauP \cite{taup}. The phases we investigate in this work are drawn with solid lines. More primary phases are plotted in order to justify the chosen epicentral distances for the sensitivity analysis, which are shown by blue squares on the solid lines. \textit{Right}: Theoretical raypaths for the same model. Red triangles denote stations at the epicentral distances were we opt observing the phases for the sensitivity analysis. The colours in the two sub-figures are not corresponding. IC denotes inner core, OC denotes outer core. Plots are made using ObsPy \citep{obspy}. }
    \label{fig:raypaths}
\end{figure}
\clearpage


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/models_and_dataset-v2}
    \caption{Dataset, and CMB topography models used in this study. Panel (a) shows the events (red stars) and stations from the Global Seismographic Network (cyan inverted triangles). Panels (b) to (e) show models T1 (b) and TC1 (c) based on the mantle convection simulations of \cite{Deschamps2018} (see main text), and LGW91 \citep{Xiang-DongLi1991} (d) and TK10 \citep{Tanaka2010} (e), inferred from actual data. Panel (f) shows the same model TK10 as panel (e), except for a change in scale of the color bar.}
    \label{fig:models}
\end{figure}
\clearpage


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/bouncing_points_all}
    \caption{Bouncing or crossing points at the CMB for the seven seismic phases used in this study, as labeled in each panel. Blue-filled circles show P phases, while red circles show S phases. For SKKS and PKKP, yellow- and green-filled circles show the underneath bouncing points at the CMB.}
    \label{fig:bouncing}
\end{figure}
\clearpage




\begin{figure}
    \centering
    \includegraphics[width=.75\textwidth, angle=0]{figures/iter_stack_ScS}
    \caption{Illustration of the adaptive stacking procedure \citep{Rawlinson2004} used to define the time windows, for the ScS phase for model S20RTS and event no. 1 in Table $\ref{tab:events}$. (a) Waveforms before alignment, using time windows 5~s before, and 20~s after the ScS arrival; (b) same as (a), but after alignment using the source wavelet (red trace) obtained from the adaptive stacking procedure.}
    \label{fig:iterstack}
\end{figure}
\clearpage


\begin{figure}
    \centering
    \includegraphics[width=\textwidth, height=0.7\textheight]{figures/Pwaves-1Dvs3D-models-RTWF}
    \caption{Comparison between ray theoretical prediction of time shift given a CMB topography model to the time anomaly measured on each time windowed seismic phase by comparing synthetic waveforms in \textcolor{red}{1-D} and \textcolor{blue}{3-D} velocity background, red and blue points on the plots, respectively. Each column corresponds to a different topography model (\emph{TK, Li, T1, TC1}). Each row corresponds to a seismic phase (\emph{PcS, PcP, PKP} and \emph{PKKP}). Most of the phases show low correspondence between predicted and measured by cross-correlation time shift, implying a loss of information when interpreting the time shift only due to topographic variation using RT.}
    \label{fig:Pwaves-1D-models-RTWF}
\end{figure}
\clearpage
\begin{figure}
    \centering
    \includegraphics[width=\textwidth, height=0.55\textheight]{figures/Swaves-1Dvs3D-models-RTWF}
    \caption{Similar as figure $\ref{fig:Pwaves-1D-models-RTWF}$. Each row corresponds to a seismic phase (\emph{ScS, SKS} and \emph{SKKS}). Most of the phases show better correspondence between predicted and measured by cross-correlation time shift, implying that S-wave phases have a better sensitivity to CMB topography and this can be accommodated by RT.}
    \label{fig:Swaves-1D-models-RTWF}
\end{figure}
\clearpage




\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth,height=0.8\textheight]{figures/scaledLi}
     \caption{ }
    \label{fig:scaledli}
\end{figure}
\clearpage




% Sensitivity kernels

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth, height=0.8\textheight]{figures/pwavesCMB}
    \caption{Fr\'echet sensitivity kernels for the group of \emph{P-}waves examined here. Each row corresponds to a phase, from left to right, the figures show: synthetic seismogram and corresponding time window isolating the phase, compressional wavespeed volumetric kernel ($V_{P}$), shear wavespeed volumetric kernel ($V_{S}$), boundary kernel on denoting the core-mantle transition. From top to bottom: \emph{PcS (53$^{\circ}$), PKP (160$^{\circ}$), PKKP (110$^{\circ}$), PcP (53$^{\circ}$)}. The units of volumetric kernels are $km^{-3} \cdot s$ and for the boundary kernels $km^{-2} \cdot s$.}
    \label{fig:pkernels}
\end{figure}
\clearpage


\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth,height=0.5\textheight]{figures/swavesCMB}
     \caption{Similar to figure $\ref{fig:pkernels}$, now for the selected \emph{S-}wave phases. From top to bottom: \emph{SKS (110$^{\circ}$), SKKS (110$^{\circ}$) and ScS (53$^{\circ}$)}. The units of volumetric kernels are $km^{-3} \cdot s$ and for the boundary kernels $km^{-2} \cdot s$.}
    \label{fig:skernels}
\end{figure}
\clearpage

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth,height=0.5\textheight]{figures/1dvs3dboundSKS.pdf}
     \caption{Comparison between the boundary kernels computed in 3-D background using model S40RTS (red line) and the same seismic phase \emph{SKS} in 1-D background PREM (black line). the fact that the boundary kernels differ due to the different background model shows that interpretation of the traveltime shift of the phases due to topography should take into account the trade-off between topography and 3-D velocity variation, ideally in a non-linear way (not only by subtracting a time shift correction due to the 3-D mantle model). The units of boundary kernels $km^{-2} \cdot s$.}
    \label{fig:1dvs3dSKS}
\end{figure}
\clearpage



%%------Histograms for distr of time shifts due to the two different parameters %


%\begin{figure}
%    \centering
%    \includegraphics[width=\textwidth]{figures/histallPhases}
%   \caption{The histograms show the distributions of traveltime delays measured at narrow windows around the predicted PREM arrival of the phases shown on each title. The effects of topography, which are multiplied by 100 for displaying purposes (orange bars), 3-D velocity variations (blue bars) and both of these (brown bars) demonstrate that the topographic effect is almost an order of magnitude smaller than than of 3-D structure.}
%    \label{fig:histallPhases}
%\end{figure}
%\clearpage



